Devlore: Device Interrupt Protection for Confidential VMs

Modern confidential computing executes sensitive computation in an abstraction called confidential VMs and protects from the hypervisor, host OS, and other co-resident VMs. It has been shown that an attacker can inject malicious interrupts to break the confidentiality and integrity of confidential VMs. We present Devlore, a device interrupt isolation mechanism that protects confidential VMs from interrupt manipulation attacks. Our design employs a delegate-but-check strategy by offloading interrupt management to the hypervisor, but adds correctness checks in the trusted software. We prototype our design on Arm Confidential Computing Architecture (CCA). We evaluate it on Arm FVP to demonstrate four diverse devices attached to confidential VMs and report costs on a Rock5b board. Our case studies show the feasibility of real-world use cases and that Devlore incurs minimal overheads of 0.06% for typical integrated GPU applications.

==> Makefile <==
PAPERNAME ?= main
BIBFILE   ?= paper

LATEX      := pdflatex
LATEXFLAGS := -interaction=nonstopmode -halt-on-error -file-line-error

.PHONY: all bib clean distclean

all:
	$(LATEX) $(LATEXFLAGS) $(PAPERNAME).tex
	@if [ -f "$(BIBFILE).bib" ]; then \
		echo "Running BibTeX using $(BIBFILE).bib"; \
		bibtex $(PAPERNAME); \
	elif [ -f "$(PAPERNAME).bbl" ]; then \
		echo "Using existing $(PAPERNAME).bbl"; \
	else \
		echo "ERROR: Neither $(BIBFILE).bib nor $(PAPERNAME).bbl exists."; \
		exit 1; \
	fi
	$(LATEX) $(LATEXFLAGS) $(PAPERNAME).tex
	$(LATEX) $(LATEXFLAGS) $(PAPERNAME).tex

bib:
	@test -f "$(BIBFILE).bib" || \
		(echo "ERROR: $(BIBFILE).bib is missing."; exit 1)
	$(LATEX) $(LATEXFLAGS) $(PAPERNAME).tex
	bibtex $(PAPERNAME)
	$(LATEX) $(LATEXFLAGS) $(PAPERNAME).tex
	$(LATEX) $(LATEXFLAGS) $(PAPERNAME).tex

clean:
	rm -f \
		$(PAPERNAME).aux \
		$(PAPERNAME).blg \
		$(PAPERNAME).log \
		$(PAPERNAME).out \
		$(PAPERNAME).toc \
		$(PAPERNAME).lof \
		$(PAPERNAME).lot \
		$(PAPERNAME).fls \
		$(PAPERNAME).fdb_latexmk \
		$(PAPERNAME).synctex.gz \
		*.ilg *.idx *.ind *.dvi *.ps *~

distclean: clean
	rm -f $(PAPERNAME).pdf $(PAPERNAME).bbl


prepare-arxiv: 
	arxiv_latex_cleaner .
